Requirements Analysis of a Quad-Redundant Flight Control System

In this paper we detail our effort to formalize and prove requirements for the Quad-redundant Flight Control System (QFCS) within NASA's Transport Class Model (TCM). We use a compositional approach with assume-guarantee contracts that correspond to the requirements for software components embedded in an AADL system architecture model. This approach is designed to exploit the verification effort and artifacts that are already part of typical software verification processes in the avionics domain. Our approach is supported by an AADL annex that allows specification of contracts along with a tool, called AGREE, for performing compositional verification. The goal of this paper is to show the benefits of a compositional verification approach applied to a realistic avionics system and to demonstrate the effectiveness of the AGREE tool in performing this analysis.

==> agree-language.tex <==
\subsection{The AGREE language}

AADL describes the interface of a component in a \textit{component type}. A component type contains a list of \textit{features}, which are the inputs and outputs of a component, and possibly a list of AADL properties.  A \textit{component implementation} is used to describe a specific instance of a component type.  A component implementation contains a set of subcomponents and set of connections that occur between its subcomponents and features.  

For example, one may decide to create a component type for a car which contains features describing its throttle, speed, and direction.  A car component may have many implementations (like a 2006 Toyota Camry, or a McLaren 650s). Different implementations may contain different electronic components, actuators, etc \ldots.

AADL contains special syntax elements called \textit{annexes} that can be used to extend the language. The syntax for a component's contract exists in an AGREE annex placed inside of the component type.  AGREE syntax can also be placed inside of annexes in a component implementation or an AADL Package. Syntax placed in an annex in an AADL Package can be used to create libraries that can be referenced by other components.  

Figure~\ref{fig:grammar} shows the simplified illustration of AGREE's grammar in BNF. An AGREE annex in an AADL component type contains syntax that is recognized as a \texttt{<contr>} element. Similarly, an AGREE annex in an AADL component implementation contains syntax that is recognized as a \texttt{<impl>} element. The types of statements found in an AADL component type are described below.

\input{grammar.tex}


\begin{itemize}
\item \textbf{Guarantee Statement}: Guarantee statements are proven by the guarantees present in subcomponent contracts.  They in turn are used to prove the guarantees of a components one step above them in the model hierarchy.  These are the guarantees described in Section~\ref{sec:comp-v}.

\item \textbf{Assume Statement}: Assume statements are used to prove the guarantees of the contract as well as the assumptions of the subcomponent contracts. These are the assumptions described in Section~\ref{sec:comp-v}. 

\item \textbf{Initially Statement}: Initially statements are used to constrain the values of the component outputs and intermediate variables before the components clock ever ticks.  This is very subtle and only matters in models that are not synchronous. These statements will make more sense when we explain how we modelled the ULB requirements in Section~\ref{sec:ulb-agree}.

\item \textbf{Equation Statement}: Equation statements are used to define variables.  Variables defined with equation statements are thought of as ``intermediate'' variables or variables that are not meant to be visible in the architectural model (unlike component outputs or inputs).  Equation statements can define variables explicitly by setting the equation equal to an expression immediately after it is defined.  Equation statements can also define variables implicitly by not setting them equal to anything, but constraining them with assumption, assertion, initially, or guarantee statements. Equation statements can actually define more than one variable at once by writing them in a comma delimited list.  One might do this to constrain a set of variables to the results of a node statement that has multiple return values or to more cleanly list a set of implicitly defined variables.

\item \textbf{Node Statement}: Node statements are used to define ``functions'' that might be used frequently in a component type or implementation.  Nodes cannot be recursive or mutually recursive.  Nodes can have multiple return values. If this is the cause, they must be referenced by an equation statement that has multiple arguments. Nodes can also be defined in an AADL Package. If so, they can be referenced in any expression anywhere in the model.  This way one can make a ``library'' of certain types of nodes that are useful for different tasks.
\end{itemize}

The \texttt{<expr>} elements in the grammar are very similar to Lustre expressions~\cite{lustre}.  Expressions reason about the current state or past states of variables and can reference variables defined in equation statements or other identifiers in the AADL model. The following is a list of different types of expressions. We describe them in the order they are listed as alternatives to the grammar rule for \texttt{<expr>} in Figure~\ref{fig:grammar}.

\begin{itemize}
\item \textbf{Boolean Literal}: \texttt{true} or \texttt{false}

\item \textbf{Integer Literal}: \texttt{1}, \texttt{42}, \texttt{1337}, etc \ldots

\item \textbf{Real Literal}: \texttt{3.1415}, \texttt{1.6180}, \texttt{0.001}, etc \ldots

\item \textbf{ID Expression}: An ID as an alpha numeric character (not starting with a number).  ID expressions can also have dots in them (e.g., \texttt{foo.bar.biz}.  ID expressions correspond to variables defined in equation statements or AADL features.  AGREE reasons about the AADL \texttt{Base\_Types::Integer}, \\\texttt{Base\_Types::Float}, and \texttt{Base\_Types::Boolean} as \texttt{int}, \texttt{real}, and \texttt{bool} types, respectively.  ID expressions with dots in them correspond to record types or variables of a subcomponent.  For example, one could use the ID expression \texttt{foo.bar} to reference the input, output, or equation variable \texttt{bar} or subcomponent \texttt{foo} within the implementation of some AADL component. AGREE reasons about AADL Data Implementations like record types.  This will be more clear when we discuss how we modelled the STANAG 4586 messages in Section~\ref{sec:ulb-agree}.

\item \textbf{Node Call Expression}: A node call expression is an ID of a defined node followed by parenthesis.  If the node is defined in an AADL Package, then the ID should be the AADL Package name a dot (\texttt{.}) and then the node name.

\item \textbf{Previous Value Expression}: A previous value expression evaluates to the value of its argument on the previous time frame.  It recommended that it be guarded by an arrow expressions as its value is undefined on the initial state.

\item \textbf{Event Expression}: An event expression is a special predicate that is used to reason about AADL event data ports.  For an input event data port, its semantics are such that it evaluates to true if a value is \textit{present} on the event port and false otherwise. For an output event data port, its semantics are such that it evaluates true if data is being sent on the port and false otherwise.

\item \textbf{Floor Expression}: A floor expression takes an expression of type \texttt{real} as an argument and returns an \texttt{int} equal to the floor of the number.

\item \textbf{Real Expression}: A real expression takes an expression of type \texttt{int} as argument and returns a \texttt{real} equal to its value.

\item \textbf{Get Property Expression}: A get property expression allows a user to reason about values of AADL properties in the model.  The first argument is the relative path to an AADL component in the instance model or `\texttt{this}' if the property exists in the component in which get property statement lives.  The second argument is the name of the AADL property.

\item \textbf{Minus Expression}: This expression is used to negate integer or real valued expressions.

\item \textbf{Not Expression}: This expression is used to negate boolean valued expressions

\item \textbf{Record Update Expression}: The record update expression expects an expression of record type on the left hand side of the curly braces.  It returns the same record as the left hand side expression except with its member ``ID'' set to the value of the expression on the right hand side of the `\texttt{:=}';

\item \textbf{Arithmetic Operations}: Arithmetic operations must be performed on expressions of the same type.  They follow the standard order of precedence.  Note that AGREE will give a warning if you write an expression that is not linear.  Some theorem provers do not reason about non-linear expressions.  Non-linear integer arithmetic is undecidable and most theorem provers do not use a decidble decision procedure for non-linear real arithmetic.  So it is recommended that you only use linear expressions.

\item \textbf{Relation Expressions}: Relation expressions can be performed on integers or reals, but not a combination of both.  Equality can be used on Booleans as well.

\item \textbf{Boolean Expressions}: Boolean expressions have the standard associative properties and order of precedence. 

\item \textbf{Arrow Expression}: The arrow expression evaluates to the value of the expression of the left hand side of the arrow on the initial time step. Otherwise it evaluates to the value of the expression on the right hand side of the arrow.  The arrow expression is used with the \texttt{pre} expression to reason about past values of variables. For example, we can define a variable in an AGREE contract that starts at zero and increments by one each step in time using an equation statement:

\begin{center}
{\color{color18} \textbf{eq}} count {\color{color18} \textbf{:}} {\color{color18} \textbf{int = }} 0 {\color{color18} \textbf{-\texttt{>}}}
{\color{color18} \textbf{pre(}} count {\color{color18} \textbf{)}} + 1
\end{center}

Note that the difference between arrow expressions and the initially statements discussed earlier is very subtle.  Before a subcomponents clock ticks the values of its outputs and intermediate variables defined by equation statements are only constrained by the expressions in initially statements.  Once the subcomponents clock ticks for the first time the expressions in the initially statements become irrelevant and all arrow expressions in the subcomponent evaluate to the value of their left hand side expression.

\end{itemize}  


While assumption and guarantee statements exclusively live in component types, component implementations exclusively contain other grammar elements. Specifically, component implementations can contain the following elements.

\begin{itemize}
\item \textbf{Synchrony Statement}: Synchrony statements describe the order in which the subcomponents execute.  Right now we support modelling systems synchronously or quasi-synchronously.  The synchrony statement expects an integer value which indicates the number of times a subcomponent's clock can tick since any other clock has ticked.  The phrase \texttt{no\_simult} can optionally be placed at the end of the statement to indicate that no two subcomponent clocks may tick simultaneously.  This would be indicative of multiple threads scheduled to run on a single processor for example.

\item \textbf{Assert Statement}: Assert statements make unchecked statements about how the component behaves.  These are also used to reference variables from a subcomponent in the component contract.  For the purpose of analysis assertions are treated just like the system assumptions in the formulas presented in Section~\ref{sec:comp-v}.  However, we never verify that the assertions actually hold.  That is to say, the assertions of a subcomponent are never proven to hold like subcomponent assumptions in Formula~\ref{fml:correct-assump}.  Assertions can be thought of as unchecked assumptions about the behavior of component. Assert statements can refer to equations or features defined in the component type. They are often used to refer to subcomponent variables in contracts higher up in the model hierarchy. We show examples of this in Section~\ref{sec:ulb-agree}.

\item \textbf{Lemma Statement}: Lemma statements are proven just like guarantees.  These are used to help the model checker learn facts to improve its ability to prove other properties.  They differ from guarantees in that subcomponent lemmas are not used to prove other subcomponent guarantees or system guarantees.  In other words, lemmas only ever appear as system guarantees on the right hand side of the implication in Formula~\ref{fml:guar-check}.
\end{itemize}

==> arch.tex <==
\section{QFCS Architecture}

\begin{figure}
\begin{center}
\includegraphics[scale=0.4]{reqs-rot.pdf}
\end{center}
\caption{The QFCS requirements hierarchy}
\label{fig:reqs-hier}
\end{figure}

==> grammar.tex <==
\begin{figure}
\begin{grammar}
<contr> ::= <contr-stmt> <contr> | <contr-stmt>

<contr-stmt> ::= `guarantee' <STR> `:' <expr> `;'
\alt `assume' <STR> `:' <expr> `;'
\alt `initially' `:' <expr> `;'
\alt <eq-stmt>
\alt <node-stmt>

<impl> ::= <impl-stmt> <impl> | <impl-stmt>

<impl-stmt> ::= `assert' <expr> `;'
\alt `synchrony' `:' <INT-LIT> (`no_simult')? `;'
\alt `lemma' <STR> `:' <expr> `;'
\alt <eq-stmt>
\alt <node-stmt>

<eq-stmt> ::= `eq' <arg-lst> `=' <expr> `;'
\alt `eq' <arg-lst> `;'

<node-stmnt> ::= `node' <ID> `(' <arg-lst> `)' \\
`returns' `(' <arg-lst> `)' `;' \\
(`var' <arg-lst>)? \\
`let' <eq-lst> `tel' `;'

<expr> ::= <BOOL-LIT>
\alt <INT-LIT>
\alt <REAL-LIT>
\alt <ID>
\alt <ID> `(' <expr-lst> `)'
\alt `pre' `(' <expr> `)'
\alt `event' `(' <ID> `)'
\alt `floor' `(' <expr> `)'
\alt `real' `(' <expr> `)'
\alt `Get_Property' `(' <expr> `,' <aadl-property> `)'
\alt `-' <expr>
\alt `not' <expr>
\alt <expr> `{' <ID> `:=' <expr> `}'
\alt <expr> (`*'|`/'|`mod'|`+'|`-') <expr>
\alt <expr> (`<'|`<='|`>'|`>='|`='|`!=') <expr>
\alt <expr> (`and'|`or') <expr>
\alt <expr> `=>' <expr>
\alt <expr> `->' <expr>

<type> ::= `int' | `real' | `bool' | <aadl-type>

<arg-lst> ::= <ID> `:' <type> `,' <arg-lst> | <ID> `:' <type>

<eq-lst> ::= <eq-stmt> <eq-lst> | <eq-stmt>

<expr-lst> ::= <expr> `,' <expr-lst> | <expr>

\end{grammar}
\caption{A simplified illustration of the grammar for AGREE}
\label{fig:grammar}
\end{figure}
